VLM as Policy: Common-Law Content Moderation Framework for Short Video Platform

Exponentially growing short video platforms (SVPs) face significant challenges in moderating content detrimental to users' mental health, particularly for minors. The dissemination of such content on SVPs can lead to catastrophic societal consequences. Although substantial efforts have been dedicated to moderating such content, existing methods suffer from critical limitations: (1) Manual review is prone to human bias and incurs high operational costs. (2) Automated methods, though efficient, lack nuanced content understanding, resulting in lower accuracy. (3) Industrial moderation regulations struggle to adapt to rapidly evolving trends due to long update cycles. In this paper, we annotate the first SVP content moderation benchmark with authentic user/reviewer feedback to fill the absence of benchmark in this field. Then we evaluate various methods on the benchmark to verify the existence of the aforementioned limitations. We further propose our common-law content moderation framework named KuaiMod to address these challenges. KuaiMod consists of three components: training data construction, offline adaptation, and online deployment & refinement. Leveraging large vision language model (VLM) and Chain-of-Thought (CoT) reasoning, KuaiMod adequately models video toxicity based on sparse user feedback and fosters dynamic moderation policy with rapid update speed and high accuracy. Offline experiments and large-scale online A/B test demonstrates the superiority of KuaiMod: KuaiMod achieves the best moderation performance on our benchmark. The deployment of KuaiMod reduces the user reporting rate by 20% and its application in video recommendation increases both Daily Active User (DAU) and APP Usage Time (AUT) on several Kuaishou scenarios. We have open-sourced our benchmark at https://kuaimod.github.io.

==> Sections/Preliminaries.tex <==
\section{PRELIMINARIES}

% \subsubsection{Model Overview}
% We propose the EVLM (Efficient Vision-Language Model), an innovative architecture designed to enhance visual understanding while maintaining high computational efficiency. Traditional vision-language models often face challenges with long visual sequences and rely on single-layer visual features, leading to significant computational overhead and incomplete visual perception. Our EVLM addresses these issues by incorporating a cross-attention mechanism for efficient image-text interaction, utilizing hierarchical ViT features to capture multi-level visual details, and introducing a Mixture of Experts (MoE) mechanism to enhance model effectiveness.

% \subsubsection{Architecture Design}
% Our EVLM architecture is built upon the Flamingo framework and consists of three main components: a visual encoder, a large language model (LLM), and a Gated Cross Attention Layer. The visual encoder employs the EVA2-CLIP-E-Plus model, from which hierarchical features are extracted and fed into the cross-attention layers. This design allows the model to perceive visual signals at different levels, aiding in understanding tasks of varying granularity. The LLM is based on Qwen-14B-Chat 1.0, known for its strong performance in content understanding and logical reasoning. To condition the LLM on visual inputs, we insert gated cross-attention layers before each transformer layer of the LLM. This ensures that the model can process visual inputs efficiently while maintaining high performance.

% \subsubsection{Training Strategy}
% The training of our EVLM model is divided into three stages: multi-modal pre-training, multi-task continual pre-training, and supervised fine-tuning. In the multi-modal pre-training stage, we focus on aligning visual and textual modalities and learning the intrinsic relationships within the data. We use a large-scale dataset of image-text pairs, with extensive data cleaning to ensure high relevance between images and text. The continual pre-training stage introduces multi-task learning, incorporating datasets from various tasks such as visual question answering (VQA), OCR, and detection. This phase enhances the model's ability to handle high-level visual reasoning tasks. Finally, the supervised fine-tuning stage activates the model's instruction-following abilities using high-quality instruction tuning data, further improving its performance in specific tasks.

% \subsubsection{Performance and Evaluation}
% Our EVLM model demonstrates superior performance on a comprehensive set of benchmarks, covering general VQA, text-oriented VQA, and general multimodal tasks. It achieves high accuracy in tasks such as ScienceQA, VQAv2, and GQA, showcasing its strong capabilities in integrating multimodal information and utilizing extensive prior knowledge for robust reasoning. Additionally, our model shows excellent performance in fine-grained visual perception tasks, such as AI2Diagram and ChartQA, highlighting its ability to comprehend complex visual details. The model's bilingual capabilities and reduced hallucinations in visual descriptions further enhance its versatility and effectiveness in handling complex visual and textual information.

\label{sec: yuanqi}
In this section, we briefly introduce \C{}'s self-developed \Y{} VLM model, which serves as the foundation model for \M{} and is used to generate \M{}'s training data.  

\subsection{Overview of \Y{} Model}

The \Y{} model is an efficient VLM following the Flamingo-style architecture, consisting of:
% \begin{itemize}
    (1) \textbf{Visual Encoder:} Built upon the EVA2-CLIP-E-Plus model, it extracts hierarchical vision features at multiple levels, enabling fine-grained perception of visual elements.
    (2) \textbf{LLM Foundation:} Based on Qwen-14B-Chat 1.0, providing strong content understanding and logical reasoning capabilities.
    (3) \textbf{Gated Cross-Attention Layers:} Inserted before each transformer layer in the LLM, allowing effective image-text fusion while maintaining high computational efficiency.
    (4) \textbf{Mixture of Experts (MoE):} Optimizes model effectiveness by dynamically activating specialized subnetworks.
% \end{itemize}

\subsection{Training \& Evaluation}
The \Y{} model undergoes a three-stage training pipeline:
% \begin{itemize}
    (1) \textbf{Multi-Modal Pre-Training:} Aligns visual and textual modalities using large-scale image-text pairs, ensuring high relevance through extensive data cleaning.
    (2) \textbf{Multi-Task Continual Pre-Training:} Incorporates tasks such as visual question answering (VQA), OCR, and object detection, enhancing high-level reasoning capabilities.
    (3) \textbf{Supervised Fine-Tuning (SFT):} Activates instruction-following abilities using high-quality instruction data.
% \end{itemize}

The hierarchical feature extraction mechanism, cross-attention architecture, and multi-stage training pipeline enable the \Y{} model to achieve state-of-the-art performance on diverse benchmarks including general  visual question answering, fine-grained visual perception, bilingual capabilities and hallucination.
% \begin{itemize}
%     \item \textbf{General and Text-Oriented VQA:} Excels on datasets like ScienceQA, VQAv2, and GQA, showcasing robust multimodal reasoning capabilities.
%     \item \textbf{Fine-Grained Visual Perception:} Demonstrates strong comprehension in complex tasks such as AI2Diagram and ChartQA.
%     \item \textbf{Bilingual Capabilities and Reduced Hallucination:} Provides more accurate visual descriptions with fewer hallucinations, enhancing reliability across different contexts.
% \end{itemize}
Overall,  \Y{} is highly suitable for tasks requiring complex visual and textual integration.


==> tables/online_1.tex <==
% \vspace{-0.1cm}
\begin{table}[h]
    \centering
    \caption{\M{}'s online A/B test results for comprehensive ecosystem governance on \C{} NEBULA and Featured.}
    % \vspace{-0.2cm}
    \resizebox{1.0\columnwidth}{!}{
        \begin{tabular}{lccc}
            \toprule
            \textbf{Column} & \textbf{Report Rate (\%) $\downarrow$} & \textbf{DAU (\%) $\uparrow$} & \textbf{Total AUT (\%) $\uparrow$} \\
            \midrule
            NEBULA & \cellcolor{green!30} -24.34 & \cellcolor{green!25} +0.016 & \cellcolor{red!5} -0.002 \\
            Featured & \cellcolor{green!20} -18.98 & \cellcolor{red!5} -0.002 & \cellcolor{green!25} +0.012 \\
            \bottomrule
        \end{tabular}
    }
    % \vspace{-0.2cm}
    \label{tab:online_exp1}
\end{table}



==> tables/online_2.tex <==
% \vspace{-0.1cm}
\begin{table}[h]
    \centering
    \caption{\M{}'s online A/B test result for personalized recommendation enhancement on \C{} Main Site}   

    \begin{tabular}{lccc}
        \toprule
        \textbf{Column} & \textbf{DAU (\%) $\uparrow$} & \textbf{Avg AUT (\%) $\uparrow$} & \textbf{Total AUT (\%) $\uparrow$} \\
        \midrule
        Main Site & \cellcolor{green!20} +0.028 & \cellcolor{green!20} +0.033 & \cellcolor{green!30} +0.063 \\
        \bottomrule
    \end{tabular}    
% \vspace{-0.2cm}
    \label{tab:online_exp2}
\end{table}
